Sampling in Combinatorial Spaces with SurVAE Flow Augmented MCMC

Hybrid Monte Carlo is a powerful Markov Chain Monte Carlo method for sampling from complex continuous distributions. However, a major limitation of HMC is its inability to be applied to discrete domains due to the lack of gradient signal. In this work, we introduce a new approach based on augmenting Monte Carlo methods with SurVAE Flows to sample from discrete distributions using a combination of neural transport methods like normalizing flows and variational dequantization, and the Metropolis-Hastings rule. Our method first learns a continuous embedding of the discrete space using a surjective map and subsequently learns a bijective transformation from the continuous space to an approximately Gaussian distributed latent variable. Sampling proceeds by simulating MCMC chains in the latent space and mapping these samples to the target discrete space via the learned transformations. We demonstrate the efficacy of our algorithm on a range of examples from statistics, computational physics and machine learning, and observe improvements compared to alternative algorithms.

==> sections/prelim.tex <==
\section{Introduction}

Markov Chain Monte Carlo (MCMC) is regularly used to generate samples from posterior distributions. The variant Hamiltonian Monte Carlo (HMC) promises better scalability and has enjoyed wide-ranging success as one of the most reliable approaches in a general setting.

However, a lack of supports for discrete domains is a fundamental limitation of HMC. This difficulty arises from the fact that the construction of HMC proposals is based on numerical solution of differential equations. In general, approximating the likelihood of a discrete random variable with a continuous function is difficult and hence has restricted the use of HMC for such domains.

In this paper, we alleviate this problem by proposing a sampler that uses SurVAE flow transport layers to map the discrete space on to a Gaussian latent space using variational dequantization and normalizing flows. We thereby employ HMC in this amenable Gaussian latent space to generate samples from the target discrete space using the learned transformations.

We will demonstrate the efficacy of our algorithm by training Bayesian quantized neural networks by using our model to sample from the posterior distribution of the quantized weights. 

\section{Preliminaries and Setup}
\label{sec:prelim}

Given access to an unnormalized density $\pi(\thetav)$ over the discrete random variable $\thetav \subseteq [K]^d := \{1, 2, 3, \cdots, K\}^d$, we want to generate $m$ samples from the density $\pi(\thetav)$. In this draft, we address this problem using neural transport maps. We begin by reviewing briefly the concepts of Neural Transport (NeuTRA) \cite{hoffman2019neutra} and variational dequantization \cite{ho2019flow++} that will be useful in our subsequent exposition.

\subsection{NeuTRA: Neural Transport}
\label{subsec:neutra}

Assume that we are given access to an unnormalized density $\pi(\thetav)$ and we want to generate samples from $\pi(\thetav)$. NeuTra proceeds in two steps: Learning and Sampling.

\paragraph{Learning:} In NeuTra, the authors proposed to learn a diffeomorphic transformation $T_{\phi}: \Zsf \to \Theta$ where $\Zsf \sim p_{\zv}$ and $p_{\zv}$ has a simple geometry. Learning proceeds by sampling $\lbag \zv_1, \ldots, \zv_n \rbag \sim p_{\zv}$ and minimizing the $\mathsf{KL}$-divergence between $\pi(\thetav)$ and the push-forward density $\tilde{\pi}(\thetav) := p_{\zv}(\zv)\cdot \Big|\nabla_{z} T_{\phi}(\zv)\Big|$ \ie \begin{align*}
    \Lc(\phi) := - \mathsf{KL}(\tilde{\pi}(\thetav)|| \pi(\thetav)) &= \int_{\thetav} \tilde{\pi}(\thetav) \log \frac{\pi(\thetav)}{\tilde{\pi}(\thetav)} \rmd \thetav \\
    & = \int_{z} p_{\zv}(\zv) \log \frac{\pi(T_{\phi}(\zv))}{p_{\zv}(\zv) \cdot \Big|\frac{\partial T_{\phi(\zv)}}{\partial \zv}\Big|^{-1}} \rmd \zv
\end{align*}
Thus, given the sample $\lbag \zv_1, \ldots, \zv_n \rbag \sim p_{\zv}$, we can learn $T_{\phi}$ by:
\begin{equation}
    \label{eq:neutra_learning}
    T_{\phi}^* := \arg \min_{\phi} \frac{1}{n}\sum_{i=1}^n \log \frac{\pi(T_{\phi}(\zv_i))}{p_{\zv}(\zv_i) \cdot \Big|\frac{\partial T_{\phi(\zv)}}{\partial \zv}\Big|_{\zv = \zv_i}^{-1}}
\end{equation}
This learning paradigm tries to ensure that the density obtained by the application of the map $T_{\phi}^{-1}$ on the density $\pi(\thetav)$ results in a density that is close to the base density $p_{\zv}(\zv)$.

\paragraph{Sampling:} Once the map $T_{\phi}$ has been learned, one can sample by running an HMC sampler with the proposal as $\tilde{p}_{\zv}(\zv) := \pi(T^*_{\phi})\cdot \Big|\frac{\partial T_{\phi}(\zv)}{\partial \zv}\Big|$ to generate samples $\{\zv_1, \zv_2, \cdots, \zv_m\}$. The map $T^*_{\phi}$ then gives the samples $\{\thetav_1, \thetav_2, \cdots, \thetav_m\}$.
\subsection{Variational Dequantization}
\label{subsec: vdq}

\begin{figure*}[t]
    \centering
    \includegraphics[width=\textwidth, keepaspectratio]{plots/dq.png}
    \caption{Variational dequantization architecture}
    \label{fig:dq}
\end{figure*}

In variational dequantization, given access to a dataset $\Theta = \{\thetav_1, \thetav_2, \cdots, \thetav_n\} \subseteq \{1, 2, \cdots, K\}^d$, we are interested in modelling the discrete distribution $\pi$ from which $\Theta$ was sampled. 
A schematic for variational dequantization is shown in \Cref{fig:dq}.

\section{Dequantized Neural Transport for Discrete Random Variables}
\label{sec:d-mcmc}
Our overall set-up in terms of transformations is similar to variational dequantization and is depicted in \Cref{fig:dq}. We also proceed in two steps, as follows:

\paragraph{Learning:} We sample $\lbag \zv_1, \ldots, \zv_n \rbag \sim p_{\zv}$ and initialize $T_{\phi}$ and $T_{\lambda}$ randomly. We thus obtain the samples $\lbag \thetav_1, \ldots, \thetav_n \rbag$ since $\thetav_i = \lfloor T_{\phi}(\zv_i) \rfloor$. 

Given $p(\xv)$ and using change of variables formula, we can approximate the density $p_{\Zsf}(\zv)$ with $\tilde{p}_{\Zsf}(\zv)$ which is given by:

\begin{align}
    \label{eq:pz}
    \tilde{p}_{\Zsf}(\zv) &= p_{\Xsf}(\xv)\cdot \Bigg|\frac{\partial T_{\phi}(\zv)}{\partial \zv}\Bigg| \\
    &= \pi(\thetav)\cdot q(\uv|\thetav) \cdot \Bigg|\frac{\partial T_{\phi}(\zv)}{\partial \zv}\Bigg|, \qquad \text{[using \Cref{eq:px} ]}
\end{align}
where $\thetav = \lfloor T_{\phi}(\zv) \rfloor$ and $\uv = \zv - \lfloor T_{\phi}(\zv) \rfloor$. Thus, given samples $\lbag \zv_1, \ldots, \zv_n \rbag \sim p_{\zv}$, we can define our learning procedure by:
\begin{align*}
    \hat{T}_{\phi}, \hat{T}_{\lambda} &:= \arg \min_{\phi, \lambda} \mathsf{KL}\Big(p(\zv) || \tilde{p}(\zv)\Big) \approx \frac{1}{n}\sum_{i=1}^n \log \frac{p(\zv_i)}{\tilde{p}(\zv_i)}
\end{align*}



Since these samples are not generated from $\pi(\thetav)$, we use a weighted average of the objective given in  for learning as below:
\begin{align}
\label{eq:learn_1}
   T_{\phi}^*, T_{\lambda}^* := \arg \max_{\phi, \lambda}~ \Eb_{\varv \sim p_{\varv}} \Bigg[ \sum_{i=1}^n \pi(\thetav_i) \cdot \log \frac{p_{\mo}(\thetav_i + T_{\lambda, \thetav_i}(\varv))}{p_{\varv}(\varv)\cdot \Bigg| \frac{\partial T_{\lambda,\thetav_i}(\varv)}{\partial \varv}\Bigg|^{-1}} \Bigg]
\end{align}

Another learning procedure can be obtained by noticing that:
\begin{align*}
    \tilde{\pi}(\thetav) := \int_{\uv} p_{\mo}(\theta + \uv) \rmd \uv = \Eb_{\uv \sim q(\uv|\thetav)} \Bigg[\frac{p_{\mo}(\theta + \uv)}{q(\uv|\thetav)}\Bigg] %\\
    %\text{thus,} \qquad \log \tilde{\pi}(\thetav) \geq \Eb_{\uv \sim q(\uv|\thetav)} \Bigg[ \log \frac{p_{\mo}(\theta + \uv)}{q(\uv|\thetav)}\Bigg]
\end{align*}
Since, the samples $\lbag \thetav_1, \ldots, \thetav_n \rbag \sim \tilde{\pi}(\thetav)$, we can alternatively minimize the reverse KL divergence \ie
\begin{equation}
    T_{\phi}^*, T_{\lambda}^* := \arg \min_{\phi, \lambda} \Eb_{\thetav \sim \tilde{\pi}} \Bigg[ \log \frac{\tilde{\pi}(\thetav)}{\pi(\thetav)}\Bigg] \approx \frac{1}{n}\sum_{i=1}^n  \log \frac{\tilde{\pi}(\thetav_i)}{\pi(\thetav_i)}
\end{equation}

%We can then aim to minimize the KL-divergence between %$\pi(\thetav)$ and $\tilde{\pi}(\thetav)$ as:
%\begin{align}
    %\mathsf{KL}(\pi(\thetav)||\tilde{\pi}(\thetav)) := \Eb_{\thetav \sim \pi(\theta)} \Bigg[ \log \frac{\pi(\thetav)}{\tilde{\pi}(\thetav)}\Bigg] \approx \sum_{i=1}^n \pi(\theta_i) \log \frac{\pi(\thetav_i)}{\tilde{\pi}(\thetav_i)}
%\end{align}


\paragraph{Sampling:} We run an MCMC/HMC sampler with the proposal (or potential) as $\tilde{p}_{\zv}(\zv) := \pi(T^*_{\phi})\cdot \Big|\frac{\partial T_{\phi}(\zv)}{\partial \zv}\Big|$ to generate samples $\{\zv_1, \zv_2, \cdots, \zv_m\}$. The map $T^*_{\phi}$ then gives the samples $\{\thetav_1, \thetav_2, \cdots, \thetav_m\}$. The learned map $T_{\phi}^*$ can be used to get a proposal (with a simple enough geometry) in the latent space (or $\zv$-space) using the given unnormalized density $\pi(\thetav)$. 


%In our setup, the density $p_{\mo}(\xv)$ is a continuous analog of $\pi(\theta)$. Thus, if we are able to generate samples $\lbag \xv_1, \cdots, \xv_n \rbag \sim p_{\mo}(\xv)$ then we can easily obtain samples $\lbag \thetav_1, \cdots, \thetav_n \rbag \sim\pi(\thetav)$ since $\thetav_i = \lfloor \xv_i \rfloor$. However, the density $p_{\mo}(\xv)$ will have several modes and hence running an HMC sampler in this space will not be effective. One alternative is that we can write $p_{\mo}(\xv)$ as a convolution of the densities $\pi(\theta)$ and $q(\uv|\theta)$ since $\xv = \thetav + \uv$ \ie



%Alternatively, we know that $p_{\mo}(\xv) = p_{\zv}(\zv) \cdot \Bigg|\frac{\partial T_{\phi}(\zv)}{\partial \zv}\Bigg|$. 
